PolarDB-IMCI: A Cloud-Native HTAP Database System at Alibaba

Cloud-native databases have become the de-facto choice for mission-critical applications on the cloud due to the need for high availability, resource elasticity, and cost efficiency. Meanwhile, driven by the increasing connectivity between data generation and analysis, users prefer a single database to efficiently process both OLTP and OLAP workloads, which enhances data freshness and reduces the complexity of data synchronization and the overall business cost. In this paper, we summarize five crucial design goals for a cloud-native HTAP database based on our experience and customers' feedback, i.e., transparency, competitive OLAP performance, minimal perturbation on OLTP workloads, high data freshness, and excellent resource elasticity. As our solution to realize these goals, we present PolarDB-IMCI, a cloud-native HTAP database system designed and deployed at Alibaba Cloud. Our evaluation results show that PolarDB-IMCI is able to handle HTAP efficiently on both experimental and production workloads; notably, it speeds up analytical queries up to $\times149$ on TPC-H (100 $GB$). PolarDB-IMCI introduces low visibility delay and little performance perturbation on OLTP workloads (< 5%), and resource elasticity can be achieved by scaling out in tens of seconds.

==> Makefile <==
FILE=imci_main

all: compile

compile:  $(FILE).tex 
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done


docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	*.fdb_latexmk *.synctex.gz


clean: docclean




==> sections/revision_letter.tex <==
\title{Response to Reviewers' Comments}
\maketitle



We thank all the reviewers for their insightful reviews and constructive comments.
We also thank the meta-reviewer for overseeing our submission.
All your comments are addressed in this version and we summarize the major changes below:

\begin{itemize}
    \item \textbf{Explain why Primo acquires exclusive locks for reads}. We have improved the overview (Section \ref{sec:primo}) to clarify this problem and show the intuition of Primo.
    \item \textbf{Improve the evaluation of watermark-based group commit}. We have added two experiments in Section \ref{sec:log_exp}: (1) evaluating the impact of the epoch/interval size on latency and crash-abort rate; (2) evaluating the impact of watermark lagging and the effectiveness of force-updating the watermark.
    \item \textbf{Add deterministic database baseline.} We have added Aria, a state-of-the-art deterministic database as a baseline. We have also added a discussion of QueCC in Section \ref{sec:related_work}.
    \item \textbf{Move less critical experiments to our technical report to save space.} 
    To accommodate the new experiments and discussions, we have to move some less critical experiments including the comparison with CLV (the original Fig 11 and a part of Sec \ref{sec:log_exp}) and the comparison with TAPIR (the original Fig 14 and Sec VI-F) to our technical report due to the space limit. Please let us know if you feel necessary to keep them in the paper.
\end{itemize}

We have highlighted all major changes in \textcolor{orange}{orange} in the revision.
In the following, 
we first address the common concerns, and then
provide responses to each individual comment.

\section*{Response to common concerns}

\stitle{Concern 1} (Meta1, R1O1, R2O1, R3O1): \textit{Acquiring exclusive locks for read operations seems unnecessary. The reviewers suggest to acquire shared locks for read operations and upgrading to exclusive locks for write operations. }\vspace{0.5em}


\vspace{1em}
\stitle{Concern 2} (Meta3, R1O4, R2O4): \textit{Lack of experimental comparison with deterministic CC such as Aria/QueCC.} \vspace{0.5em}

\vspace{1em}
\stitle{Concern 3} (R1O5, R2O3): \textit{Experiments are needed to verify the claim that latency and crash-abort rate are controllable by tuning the epoch size.} \vspace{0.5em}


\section*{Response to meta-reviewer (Meta)}

\stitle{Meta1:} \textit{``acquiring exclusive locks for reads (which is odd, some CC variants acquire read locks for writes, then upgrade to exclusive during certification, but getting exclusive locks for reads seems confusing)''} \vspace{0.5em}


\vspace{1em}
\stitle{Meta2:} \textit{``impacts of watermark blocking performance''}


\vspace{1em}
\stitle{Meta3:} \textit{``lack of comparison with deterministic CC approaches such Aria/QueCC (both are cited)''} \vspace{0.5em}


\vspace{1em}
\stitle{Meta4:} \textit{``improving evaluation analysis and discussion''} \vspace{0.5em}


\section*{Response To Reviewer 1 (R1)}
\stitle{R1O1:} \textit{``It is unclear why a transaction needs to acquire exclusive locks for read operations to avoid 2PC, which seems to be the main idea of this paper.

\vspace{1em}
\stitle{R1O2:} \textit{``The authors design the concurrency control protocol based on the assumption that read operations acquire exclusive locks. Hence, the proposed method using Tictoc to reduce the lock cost seems redundant.''} \vspace{0.5em}


\vspace{1em}
\stitle{R1O3:} \textit{``A transaction may block when accessing a partition whose watermark lags behind. Although a force update of the watermark can alleviate this problem, an experimental analysis of how the blocking affects performance and how the watermark updating performs is necessary.''} \vspace{0.5em}
\vspace{1em}
\stitle{R1O4:} \textit{``The authors should conduct an experimental comparison with deterministic approaches like Aria [17]. This is because, like the proposed method, Aria does not require prior knowledge of read/write sets as well. Besides, Aria can achieve transaction reordering while the proposed method seems cannot.''} \vspace{0.5em}

\vspace{1em}
\stitle{R1O5:} \textit{``The authors argue the drawbacks, including increased latency and extra aborts, can be controlled by the size of the epochs. However, there lacks an experimental analysis by varying the epoch size to verify this statement.''} \vspace{0.5em}


\vspace{3em}
\section*{Response to Reviewer 2 (R2)}
\stitle{R2O1:} \textit{``acquiring exclusive locks for all read operations is not necessary to ensure no abort in the commit phase.

\vspace{1em}
\stitle{R2O2:} \textit{``The authors design a concurrency control algorithm by integrating TicToc to reduce locking overhead. However, because exclusive locks seem unnecessary for read operations, I am not clear about the novelty of the proposed algorithm.''} \vspace{0.5em}

\vspace{1em}
\stitle{R2O3:} \textit{``As pointed out by the authors, the proposed protocol has drawbacks like increased latency and extra aborts when failures occur. The authors claim controlling the size of the epochs can alleviate these drawbacks. However, I fail to find corresponding experiments to verify whether this statement is true.
I’d like to see experimental results of the abort rate and transaction latency by varying the epoch size.''} \vspace{0.5em}


\vspace{1em}
\stitle{R2O4:} \textit{``Experimental comparisons with deterministic approaches like Aria [17] are missing. These comparisons are necessary because Aria does not require prior knowledge of read/write sets, which is the same as the proposed method.''} \vspace{0.5em}


\section*{Response to Reviewer 3 (R3)}
\stitle{R3O1:} \textit{``It appears that acquiring X-lock for all reads is not necessary to make sure no abort in the commit phase. What would matter is to acquire locks for writes in the execution phase. This won't introduce extra X-locks but only increase the time a lock is held. Then there is no need to separate local and distributed modes, which adds system complexity and it is hard to reason about the correctness of combining WCF and OOC. If there is no extra X-lock, OOC is not needed so the extra work of handling timestamp to satisfy R1R2 in WM can be removed.''} \vspace{0.5em}

\vspace{1em}
\stitle{R3O2:} \textit{``When comparing with other systems, the author tunes all protocols to have \textasciitilde10 ms latency. However, Fig 4, 5 (c) shows that Primo has lower latency while the others have almost the same higher latency. Justifying why this is observed would be helpful.''} \vspace{0.5em}

\vspace{1em}
\stitle{R3O3:} \textit{``For Fig 4,5 (b), It would be better to show the throughput instead of improvement, so we can compare Primo w/o WM\&WCF with 2PL easier. The improvement ratio can be reported in the text. Also, there is a typo "WAF" on the x-axis.''} \vspace{0.5em}

\vspace{1em}
\stitle{R3O4:} \textit{``The idea of holding x-locks during the execution for read and write operations suggests that the proposed work may be better aligned with literature that does not separate between read and write locks. For example, work that ensures mutual exclusion or general atomic broadcast. A discussion and comparison with such methods would help understand the trade-offs in the work.''} \vspace{0.5em}

\vspace{1em}
\stitle{R3O5:} \textit{``The restrictions that are introduced due to the proposed model need to be clarified and discussed. For example, it appears that clients/coordinator unilateral aborts are not possible. For example, if the messages are sent to the participants and they all respond positively, but the user/server/coordinator unilaterally aborts then fail (which is permissible in 2PC), what are the implications of such a scenario in the proposed algorithm? Specifically, how is recovery performed for this scenario and would this lead to not allowing such unilateral aborts?''} \vspace{0.5em}

\vspace{1em}
\stitle{R3O6:} \textit{``The proposed methods would be efficient in a specific type of workload where there are no long-running read-only (or read-mostly) transactions and where the percentage of reads is not high in comparison to writes.''} \vspace{0.5em}


